Thread-modular Analysis of Release-Acquire Concurrency

We present a thread-modular abstract interpretation(TMAI) technique to verify programs under the release-acquire (RA) memory model for safety property violations. The main contributions of our work are: we capture the execution order of program statements as an abstract domain, and propose a sound upper approximation over this domain to efficiently reason over RA concurrency. The proposed domain is general in its application and captures the ordering relations as a first-class feature in the abstract interpretation theory. In particular, the domain represents a set of sequences of modifications of a global variable in concurrent programs as a partially ordered set. Under this approximation, older sequenced-before stores of a global variable are forgotten and only the latest stores per variable are preserved. We establish the soundness of our proposed abstractions and implement them in a prototype abstract interpreter called PRIORI. The evaluations of PRIORI on existing and challenging RA benchmarks demonstrate that the proposed technique is not only competitive in refutation, but also in verification. PRIORI shows significantly fast analysis runtimes with higher precision compared to recent state-of-the-art tools for RA concurrency.

==> figures/trans-dep-ex1.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{tikzpicture}[x=1em,y=1em,yscale=-1,xscale=-1]
\tikzstyle{every node}=[font=\small]


\end{tikzpicture}

==> section/algs.tex <==
\begin{figure*}[t]
\begin{minipage}[b]{0.4\textwidth}
\begin{algorithm}[H]%\small
	\DontPrintSemicolon
	\LinesNumbered
	\SetKwFunction{FThrMod}{ThreadModularAnalysis}
	\SetKwFunction{FFeasInterf}{GetInterfs}
	\SetKwFunction{FSeqAbs}{SeqAI}
	\SetKwProg{Fn}{Function}{:}{}
	\KwData{$ \mathtt{Tid} $ is the set of threads in the program}
	\Fn{\FThrMod{$ \mathtt{Tid} $}} {
		\tcp{Initialization}
		%		$ \mathcal{S} \leftarrow \phi $\;
		$ \sigma \leftarrow \phi $\;
		$ \mathcal{I} \rightarrow $ \FFeasInterf{$ \mathtt{Tid} $} \;
		\Repeat{$ \mathcal{S} = \sigma $}{
			$ \mathcal{S} \leftarrow \sigma $\;
			\ForEach{$ t \in \mathtt{Tid} $}{
				$ \sigma \leftarrow \sigma\ \squplus\ $\FSeqAbs{$ t, \mathcal{S}, \mathcal{I}(t) $}
			}
		}
	}
	\caption{TMAI}
	\label{alg:thread-modular}
\end{algorithm}
\end{minipage}
\begin{minipage}{0.59\textwidth}
	\begin{algorithm}[H]%\small
		\DontPrintSemicolon
		\LinesNumbered
		\SetKwFunction{FSeqAbs}{SeqAI}
		\SetKwFunction{FThrMod}{ThreadModularAnalysis}
		\SetKwFunction{FFeasInterf}{GetFeasibleInterfs}	
		\SetKwData{WL}{WL}
		\SetKwProg{Fn}{Function}{:}{}
		\KwData{$ t \in \mathtt{Tid} $, the thread to be analyzed \\
			\quad \quad \quad $ \mathcal{S}:$ set of explored program states \\ 
			\quad \quad \quad $ I: $ set of interferences for thread $ t $ %such that $ \forall \ld \in t$, $I(\ld) \defeq $ \\
			%\quad \quad \quad \quad $ ctx \cup \{ \st \mid \st \in t' \neq t \andspace \nppo{\st}{\ld} \andspace \nppo{\ld}{\st} \} $
			%		\quad \quad \quad $ I: \mathtt{Ld}_t \rightarrow ctx \cup \{ \st \mid \st $ is a valid interference for the load operation $ \} $ a set of interferences for thread $t$
		}
		\Fn{\FSeqAbs{$ t, \mathcal{S}, I $}} {
			\tcp{Initialize the program state}
			\For{$n \in t$}{
				\lIf{$ n \in Entry(t)$ }{$ \mathcal{S}(n) \leftarrow \top $}
				%			\modified{\lElseIf{$n \in Entry(t)$}{$\mathcal{S}(n) \leftarrow \unionof{n' \in pre(n)}{}\mathcal{S}(n')$ }}
				\lElse{$ \mathcal{S}(n) \leftarrow \bot $}
			}
			\WL $ \leftarrow Entry(t) $\;
			\While{$\exists n \in$ \WL}{
				\WL $ \leftarrow $ \WL $ \setminus \{n\} $\;
				\tcp{transfer function, \textsection \ref{subsec:sem-ra}}
				\modified{$ e \leftarrow \semof{n} (\mathcal{S}, I) $}\;
				\ForEach(){$ n' \in Succ(n) $ s.t. $ e \nsqsubseteq \unionof{n'' \in pre(n')}{}\mathcal{S}(n'') $} {
					\WL $ \leftarrow $ \WL $ \cup\ \{n'\} $ 
				}
			}
			\KwRet{$ \mathcal{S} $}
		}
		\caption{Sequential AI}
		\label{alg:seq-abs-mod}
	\end{algorithm}
\end{minipage}
\end{figure*}
%\begin{wrapfigure}[13]{r}{0.48\textwidth}
%%	\vspace{-0.5cm}
%	\begin{algorithm}[H]%\small
%		\DontPrintSemicolon
%		\LinesNumbered
%		\SetKwFunction{FThrMod}{ThreadModularAnalysis}
%		\SetKwFunction{FFeasInterf}{GetInterfs}
%		\SetKwFunction{FSeqAbs}{SeqAI}
%		\SetKwProg{Fn}{Function}{:}{}
%		\KwData{$ \mathtt{Tid} $ is the set of threads in the program}
%		\Fn{\FThrMod{$ \mathtt{Tid} $}} {
%			\tcp{Initialization}
%			%		$ \mathcal{S} \leftarrow \phi $\;
%			$ \sigma \leftarrow \phi $\;
%			$ \mathcal{I} \rightarrow $ \FFeasInterf{$ \mathtt{Tid} $} \;
%			\Repeat{$ \mathcal{S} = \sigma $}{
%				$ \mathcal{S} \leftarrow \sigma $\;
%				\ForEach{$ t \in \mathtt{Tid} $}{
%					$ \sigma \leftarrow \sigma\ \squplus\ $\FSeqAbs{$ t, \mathcal{S}, \mathcal{I}(t) $}
%				}
%			}
%		}
%		\caption{TMAI}
%		\label{alg:thread-modular}
%	\end{algorithm}
%\end{wrapfigure}


==> section/discussion.tex <==
Our current approach does not use relational interferences 
\cite{Mine-VIMCAI17,SuzanneMine-APLAS18}. %% hence, cannot take full advantage 
%% of relational domains. 
The use of relational interferences will certainly
compliment \tool's analysis when run with the octagon domain.
%%%%%%

%%%%%%
\tool can be used for TSO programs in its current form since behavior under 
TSO are a subset of behaviors under the RA memory model.
The RMO (relaxed memory model)
memory model, however,  does not guarantee the ordering between the stores of 
same variable; it only guarantees ordering between {\em dependent} operations. 
%% can only forget older dependent writes from the 
%% same thread. It will be interesting to see if that is sufficient to have a 
%% sound and precise analysis for RMO memory model.
Therefore, a relevant research direction will be to extend the proposed
partial order based TMAI   
to other memory models such as RMO.
%
Recall that for precision all the rmw events in the PO domain were
preserved.  In this context a relevant research question is
whether we can efficiently discover the set of critical store
operations for a given memory model and forget them? A solution to
this question will provably preserve the precision, while 
enabling the scalability of the analysis to larger benchmarks.

%
%% An intuitive way of explaining PSO memory model is that the store 
%% instructions of same variable and their dependent instructions are totally 
%% ordered. Hence, a simple extension of our poset based approach for PSO might 
%% include one poset per variable (same as discussed in present work) and  
%% changing the semantics of load operations to carry the dependencies of only 
%% interfering variable rather than of all the global variables. The second 
%% level of abstraction here will be limited to forgetting older dependent 
%% store instructions from the thread. 
%
%
%% It will be interesting to see how poset domain can be used to analyze other 
%% memory ordering constraints provided by C/C++11 and non-multi copy atomic 
%% architectures such as POWER and ARM.

% counter-example guided to see what to abstract
%% As discussed in \textsection\ref{subsec:improve}, we can improve the 
%% precision of the proposed approach by identifying the critical store 
%% instructions. 
%% In fact, these critical instructions need not be restricted to 
%% store instructions; any program instruction identified as critical 
%% can be a part of partial orders. The proposed approach considers 
%% latest writes per variable and all rmw instructions as critical, 
%% while all other instructions as non-critical. 
%% If we have a way to distinguish critical and non-critical 
%% program instructions based of the property of interest, 
%% the precision and efficiency of the approach 
%% can be increased many-folds. One way to find such instructions is 
%% to design an counter-example guided analysis that initially 
%% considers all instructions as non-critical and then iteratively 
%% finds critical instructions until the property is either 
%% disproved or proved. 


==> section/extra.tex <==
Running Ex
\begin{minipage}{.49\textwidth}
	\centering \footnotesize
	\fbox{\begin{tabular}{l||l||l||l}
			$a: x=1$ & $b:$ if $R(x)$  		 & $f: r_2=R(z)$ & $i: z=1$\\
			& $c: \hspace{1em} x=2$ & $g: r_3=R(y)$ & \\
			& $d: \hspace{1em} y=2$ & $h: r_4=R(x)$ & \\
			& $e: \hspace{1em} r_1=R(z)$ &  & \\
			\multicolumn{4}{c} {$P_{true}: r_3=2 \implies r_4=2 $} \\
			\multicolumn{4}{c} {$P_{false}: r_1=0 \andspace r_2=1 \implies r_4 \neq 0 $} \\
	\end{tabular}}
	\caption{Running Example: ???}
	\label{fig:running-ex}
\end{minipage}

Running example relations
\begin{figure}
	\begin{minipage}{0.49\textwidth}
		\centering \footnotesize
		\fbox{\input{figures/running-ex-true.tex}}
		\caption{HB over Running example for $P_{true}$}
		\label{fig:running-ex-true}
	\end{minipage}
	\begin{minipage}{0.5\textwidth}
		\centering \footnotesize
		\fbox{\input{figures/running-ex-false.tex}}
		\caption{HB over Running example for $P_{false}$}
		\label{fig:running-ex-false}
	\end{minipage}
\end{figure}

Explanation for running example:
The store instruction \texttt{c} will update the poset and value of variable $x$ to $ \poordered{a,c} $ and 2, respectively, resulting in program state 
$ \progstate{\poordered{a,c}, \pounordered{}, \pounordered{}}{2,0,0} $ at 
instruction \texttt{c}. Similarly, store instruction \texttt{d} will update 
the program state to $ \progstate{\poordered{a,c}, \pounordered{d}, \pounordered{}}{2,2,0} $. 
Further, when instruction \texttt{e} reads from $ self $, the program state 
remains unchanged. 
%
Let us consider interference combination $ (\rf{i}{f}, \rf{self}{g}, \rf{self}{h}) $. The interference from instruction \texttt{i} to instruction \texttt{f} will update the program state of \texttt{f} to 
$ \progstate{\pounordered{}, \pounordered{}, \pounordered{i}}{0,0,1} $. 
Since all the other instructions are reading from $ self $ in the 
interference combination, it will remain same for instructions \texttt{g} 
and \texttt{h}. This analysis results in HB relations of fig 
\ref{fig:running-ex-false} and invalidates the property $ P_{false} $.
%
Next we consider the interference combination $ (\rf{i}{f}, \rf{d}{g}, 
\rf{a}{h}) $. The interference $ \rf{i}{f} $ will result in same program 
state as explained above, i.e., $ \progstate{\pounordered{}, \pounordered{}, 
	\pounordered{i}}{0,0,1} $. Next, we analyze instruction \texttt{g} and apply 
the interference from the program state of \texttt{d} 
($ \progstate{\poordered{a,c}, \pounordered{d}, \pounordered{}}{2,2,0} $) to 
load instruction \texttt{g}. According to the proposed analysis for RA, this 
will results in join of the two program state and hence the resulting 
program state will be $ \progstate{\poordered{a,c}, \pounordered{d}, \pounordered{i}}{2,2,1} $. 
Further, the analysis of instruction \texttt{h} under interference 
combination $ \rf{a}{h} $ will try to join the program state of \texttt{a} 
with current program state. Note that, in current program state, instruction 
\texttt{a} is already a part of poset representing variable $ x $. 
Intuitively it means that the instruction \texttt{a} have already been 
executed and all of its effects have already taken place. Hence, the 
interference cannot be applied here, resulting in $ \bot $ (unreachable) 
program state at instruction \texttt{h} for this interference combination. 
%
Another interference combination $ (\rf{i}{f}, \rf{d}{g}, 
\rf{self}{h}) $, will result in same analysis until instruction \texttt{g}.
Since instruction \texttt{h} has no interfering instruction in this 
combination, the same will remain same. All reachable program states at 
instruction \texttt{h} will follow the satisfy $ P_{true} $. Since our analysis is considering all possible interference combinations, it will 
cover all possible executions. Hence, we can say that a property satisfied 
by all reachable program states at any of program location, is a valid 
property.



Analysis of \ref{fig:running-ex} without interference combinations.
\begin{figure}{}
	\fbox{
	\begin{minipage}{.2\textwidth}
		\centering \tiny
		Iteration 1:
		\begin{align*}
		\Sigma(a) = & \progstate{\pounordered{a}, \pounordered{}, \pounordered{}}{1,0,0} \\
		\Sigma(b) = & \progstate{\pounordered{}, \pounordered{}, \pounordered{}}{0,0,0} \\
		\Sigma(c) = & \bot \\
		\Sigma(d) = & \bot \\
		\Sigma(e) = & \bot \\
		\Sigma(f) = & \progstate{\pounordered{}, \pounordered{}, \pounordered{}}{0,0,0} \\
		\Sigma(g) = & \progstate{\pounordered{}, \pounordered{}, \pounordered{}}{0,0,0} \\
		\Sigma(h) = & \progstate{\pounordered{}, \pounordered{}, \pounordered{}}{0,0,0} \\
		\Sigma(i) = & \progstate{\pounordered{}, \pounordered{}, \pounordered{i}}{0,0,1} \\
		\end{align*}
	\end{minipage}
	\begin{minipage}{.33\textwidth}
		\centering \tiny
		Iteration 2:
		\begin{align*}
		\Sigma(a) = & \mathrm{-same-} \\
		\Sigma(b) = &
		\begin{cases}
			\progstate{\pounordered{}, \pounordered{}, \pounordered{}}{0,0,0}, & [\text{From self}] \\
			\progstate{\pounordered{a}, \pounordered{}, \pounordered{}}{1,0,0} & [\text{From a}]\\
		\end{cases} \\
		\Sigma(c) = & \progstate{\pounordered{\poordered{a,c}}, \pounordered{}, \pounordered{}}{2,0,0} \\
		\Sigma(d) = & \progstate{\pounordered{\poordered{a,c}}, \pounordered{d}, \pounordered{}}{2,2,0} \\
		\Sigma(e) = &
		\begin{cases}
			\progstate{\pounordered{\poordered{a,c}}, \pounordered{d}, \pounordered{}}{2,2,0}, & [\text{From self}] \\
			\progstate{\pounordered{\poordered{a,c}}, \pounordered{d}, \pounordered{i}}{2,2,1} & [\text{From i}] \\
		\end{cases} \\
		\Sigma(f) = &
		\begin{cases}
			\progstate{\pounordered{}, \pounordered{}, \pounordered{}}{0,0,0}, & [\text{From self}] \\
			\progstate{\pounordered{}, \pounordered{}, \pounordered{i}}{0,0,1} & [\text{From i}] \\
		\end{cases} \\
		\Sigma(g) = &
		\begin{cases}
			\!\begin{rcases}
				\progstate{\pounordered{}, \pounordered{}, \pounordered{}}{0,0,0} \\
				\progstate{\pounordered{}, \pounordered{}, \pounordered{i}}{0,0,1}  
			\end{rcases} 
			& [\text{From self}] \\
			\bot & [\text{From d}] \\
		\end{cases} \\
		\Sigma(h) = & 
		\begin{cases}
			\!\begin{rcases}
				\progstate{\pounordered{}, \pounordered{}, \pounordered{}}{0,0,0} \\
				\progstate{\pounordered{}, \pounordered{}, \pounordered{i}}{0,0,1}  
			\end{rcases} 
			& [\text{From self}] \\
			\!\begin{rcases}
				\progstate{\pounordered{a}, \pounordered{}, \pounordered{}}{1,0,0} \\
				\progstate{\pounordered{a}, \pounordered{}, \pounordered{i}}{1,0,1}  
			\end{rcases}
			& [\text{From a}] \\
			\bot & [\text{From c}] \\
		\end{cases} \\
		\Sigma(i) = & \mathrm{-same-} \\
		\end{align*}
	\end{minipage}
	\begin{minipage}{.4\textwidth}
		\centering \tiny
		Iteration 3:
		\begin{align*}
		\Sigma(a) = & \mathrm{-same-} \\
		\Sigma(b) = & \mathrm{-same-} \\
		\Sigma(c) = & \mathrm{-same-} \\
		\Sigma(d) = & \mathrm{-same-} \\
		\Sigma(e) = & \mathrm{-same-} \\
		\Sigma(f) = & \mathrm{-same-} \\
		\Sigma(g) = &
		\begin{cases}
			\!\begin{rcases}
				\progstate{\pounordered{}, \pounordered{}, \pounordered{}}{0,0,0} \\
				\progstate{\pounordered{}, \pounordered{}, \pounordered{i}}{0,0,1}  
			\end{rcases} 
			&[\text{From self}] \\
			\!\begin{rcases}
				\progstate{\pounordered{\poordered{a,c}}, \pounordered{d}, \pounordered{}}{2,2,0} \\
				\progstate{\pounordered{\poordered{a,c}}, \pounordered{d}, \pounordered{i}}{2,2,1}  
			\end{rcases} 
			& [\text{From d}] \\
		\end{cases} \\
		\Sigma(h) = & 
		\begin{cases}
			\!\begin{rcases}
				\progstate{\pounordered{}, \pounordered{}, \pounordered{}}{0,0,0} \\
				\progstate{\pounordered{}, \pounordered{}, \pounordered{i}}{0,0,1} \\
				\progstate{\pounordered{\poordered{a,c}}, \pounordered{d}, \pounordered{}}{2,2,0} \\
				\progstate{\pounordered{\poordered{a,c}}, \pounordered{d}, \pounordered{i}}{2,2,1} 
			\end{rcases} 
			& [\text{From self}] \\
			\!\begin{rcases}
				\progstate{\pounordered{a}, \pounordered{}, \pounordered{}}{1,0,0} \\
				\progstate{\pounordered{a}, \pounordered{}, \pounordered{i}}{1,0,1}  
			\end{rcases}
			& [\text{From a}] \\
			\!\begin{rcases}
				\progstate{\pounordered{\poordered{a,c}}, \pounordered{}, \pounordered{}}{2,0,0} \\
				\progstate{\pounordered{\poordered{a,c}}, \pounordered{}, \pounordered{i}}{2,0,1}  
			\end{rcases}
			& [\text{From c}] \\
		\end{cases} \\
		\Sigma(i) = & \mathrm{-same-} \\
		\end{align*}
	\end{minipage}}
	\caption{Running Example: ???}
	\label{fig:running-ex-working}
\end{figure}

Older sound over approximation proof
\begin{theorem} \label{thm:abspo-sound}
	$ \abs{\alpha} $ produces a sound overapproximation of $ (\mathcal{P}, \leqlattice, \join, \meet, \bot, \top) $ with respect to the RA semantics in the lattice $\abs{\mathcal{P}}$ .
\end{theorem}
\svs{Shouldn't a Galois connection to be established here?}
%\begin{proof}
As per the RA semantics, if an instruction $ {op_1} $ from thread $ t_1 $ observes the side-effects of some instruction $ {op_2} $ from thread $ t_2 $, $ {op_1} $ also observes the side-effects of everything that is  \emph{sequenced-before} $ {op_2} $ in $ t_2 $.
%	Since the thread local operations do not change the modification order, we can exclude them from this discussion and focus on the semantics of operations given in figure \ref{fig:con-sem}.

%	$ \semof{\instlab{s}: \store{x}{v}} $ appends the instruction $ s $, and removes any store or update instruction $ s' $ of variable $ x $ in $ mo $ such that $ \seqb{s'}{s} $. It also updates the $ m $ to $ m' $ with the effects of store instruction $ s $. 
%	Note that $ \semof{\instlab{s}: \store{x}{v}} $ modifies $ \mathtt{MO} $ only for variable $ x $.
%
Let a program behavior is possible only if some instruction $ l $ sees an store or update instruction $ s' $ and its effect; but due to some later store or update instruction $ s $ from the same thread, these effects are not visible to $ l $.
Such a behavior is possible in following cases:
\begin{description}
	\item [$ l $ is a load instruction and $ \rf{s'}{l} $:] If a behavior is possible only if $ \rf{s'}{l} $, our analysis will have a an interference combination with this constraints. Hence our analysis will analyze such behavior.
	
	\item[$ l $ is a load instruction and $ \seqb{s'}{s} \andspace \rf{s}{l} $:] Since $ s $ and $ s' $ are stores of the same variable from the same thread, the side-effects of $ s' $ are accumulated in the program state at program location $ s $. Hence, in such cases $ l $ will see the side-effects of an \emph{older} write.
	
	\item[$ l $ is a load instruction and $ \seqb{s''}{s'} \andspace \rf{s''}{l} $:] Since $ l $ reads from $ s'' $, the effects of store operation $ s' $ are not visible to $ l $ yet in current trace. If there is some other trace, which sees these effects (i.e. another trace with $ \rf{s'}{l} $), our analysis will analyze an interference combination having these reads-from relations.
	
	\item[$ l, l' $ are load instructions and $ \seqb{l'}{l} \andspace \rf{s}{l'} \andspace \seqb{s'}{s} $:] 
	Since $ l' $ read from $ s $, all the program state at $ s $ ($ \Sigma(s) $) will be carried to $ l' $, and hence, to $ l $. Therefore, $ l $ can observe all possible side-effects of $ s' $ in such a case.
\end{description}

Hence, any load instruction that reads from $ s $ will see the instruction $ s $ in $ mo' $ and its effects in $ m' $. 
Since the newer store instruction overwrites the older effects in memory, it is safe to remove instruction $ s' $ and its effects from the $ \Sigma(\instlab{s}) $. \qed

%	The RA semantics ensures that whenever a load operation $ l $ reads from some store operation $ s $, everything that happens-before $ s $, is also happens-before $ l $.
%	$ \semof{\instlab{l: \load{x}}} $ performs $ \join $ and $ \append $ operation over $ \mathtt{MO} $. 
%	It can remove some instructions $ op_1 $ from $ mo_l $ if and only if $ mo_s $ has an instruction $ op_2 $ such that $ \seqb{op_1}{op_2} $. 
%	In such cases, the effects of instruction $ op_1 $ will be overwritten by instruction $ op_2 $; hence, it is safe to remove instruction $ op_1 $ from the $ mo' $.
%	
%	The semantics of $ \semof{\instlab{u}: \rmwinst{x}{v}{v'}} $ performs a load operation followed by a store operation. 
%	As explained above the semantics of load operation adheres to the RA memory model.
%	Since instruction $ \instlab{u} $ updates a new value to the memory, the effects of another store or update instruction $ \instlab{s} $ will be overwritten if $ \seqb{s}{u} $. 
%	Hence, it is safe to remove such instructions $ s $ from $ \mathtt{MO} $ at $ \Sigma(\instlab{u}) $.

%\end{proof}


==> section/improve.tex <==
\subsection{Improving precision using RMW operations}
We can consider atomic read-modify-write ($ \rmw $) as both read and write operations. 
An operation $ rmw_l $ from thread $ t_1 $ reading from another $ rmw_s $ from thread 
$ t_2 $ results in synchronization of the thread $ t_1 $ with the thread $ t_2 $. 
The semantics shown in figure \ref{fig:con-sem}, performs the synchronization by 
carrying the environment at $ rmw_s $ to the instruction $ rmw_l $.

The modification order of a memory location also consists all the $ \rmw $ operations 
over the memory location. Hence, in an execution, all the $ \rmw $ operation of a 
memory location have an total order. Most of mutual exclusion benchmarks, when 
modified for the RA memory model, uses $ \rmw $ operations as synchronization fences.
Hence, we identified $ \rmw $ operations as critical operations and updated the 
semantics given in fig \ref{fig:con-sem} to (i) not delete older $ \rmw $ operation 
from $ \modord{x} $, and (ii) consistent check of two elements $ \abs{p_1}=
(\abs{\modord{x}^1}, \abspomo{\modord{x}^1}) $ and $ \abs{p_2}=(\abs{\modord{x}^2}, 
\abspomo{\modord{x}^2}) $ returns true iff $ \abs{p_1} \iscons \abs{p_2} \andspace 
\forall rmw_1 \in \abs{p_1}, rmw_2 \in \abs{p_2}, ((rmw_1, rmw_2) \in 
\abspomo{\modord{x}^1} \orspace (rmw_1, rmw_2) \in \abspomo{\modord{x}^2} 
\orspace (rmw_2, rmw_1) \in \abspomo{\modord{x}^1} \orspace (rmw_2, rmw_1) \in 
\abspomo{\modord{x}^2} ) $. The first updation keeps the identified critical 
operations in modification order, and the second updation makes sure to not combine
two modification orders that are not consistent with respect to identified 
critical operations.

%\subsection{Eager Pruning of Infeasible Interferences}
%In a thread $ t $ with $ |\mathtt{Ld}| $ load operations, each of these can 
%reads from $ |\mathtt{St}| $ store operations, the number of all possible 
%interference combination is $ O(|\mathtt{St}|^{|\mathtt{Ld}|}) $. 
%%Clearly, the number of interference combinations grow exponentially with the number 
%%of loads in a thread. 
%Clearly, in a thread with $ \sim10 $ load operations, computing all possible 
%interference combinations is resource intensive. Since some of these interference 
%combinations will be infeasible, the computation is wasteful. Hence, we modified 
%our approach to prune the infeasible interference combinations eagerly.

==> section/interf.tex <==
A load operation can take its value from program state of a store operation of a different thread or from program state of current thread.
Thread-modular analysis uses interferences to capture these reads-from relations.

One of the drawbacks of thread-modular abstract interpretation analysis is that 
it loses relationship among interferences coming from other threads. It is 
often the case that an interference $i_1$ can not change the program 
state of thread $t$ if some interference $i_2$ has already taken place during 
the execution; or interference $i_2$ is possible only if $i_1$ has already taken 
place. Classic thread modular analysis is imprecise to consider such cases. 
Example given in Figure-\ref{fig:why-ic} shows one such 
case. Here, interference from store instruction $a$ to load instruction $d$ is 
one feasible interference. But if the store instruction $b$ interferes with load 
instruction $c$, store instruction $a$ cannot interfere with load instruction 
$d$ according to the RA semantics. Hence, we modify thread-modular analysis to rectify such issues. 

\begin{figure}
	\begin{minipage}{.47\textwidth}
		\centering
		\newcolumntype{C}{>{\centering\arraybackslash}p{2.6cm}}
		\begin{tabular}{C||C}
			$a: x = 1$ 	& $c: R(x)$ \\
			$b: x = 2$ 	& $d: R(x)$ \\
			\multicolumn{2}{c} {Property: $c=2 \Rightarrow d \neq 1$} \\
		\end{tabular}
		\caption{Requirement of Feasibility Analysis}
		\label{fig:why-ic}
	\end{minipage}
	\begin{minipage}{.47\textwidth}
		\centering
		\newcolumntype{C}{>{\centering\arraybackslash}p{2.6cm}}
		\begin{tabular}{C||C}
			$a: x = 1$ 	& $b: R(x)$ \\
						& $c: R(x)$ \\
			\multicolumn{2}{c} {$ [\rf{a}{b}, \rf{a}{c}] \in \mathcal{IC}(t_2) $} \\
		\end{tabular}
		\caption{Redundant Interference}
		\label{fig:red-interf}
	\end{minipage}
\end{figure}

%%% example to highlight need of interference combinations
We borrow the idea of using interference combinations proposed in 
\citep{KusanoWang-FSE16,KusanoWang-FSE17} to make the analysis flow-sensitive. 
However, our technique is more efficient in generating and applying 
these interference combinations. We create all possible interference 
combinations and try to filter out the infeasible combination by performing 
\emph{sequenced-before}($\seqb{}{}$) and \emph{reads-from}($\rf{}{}$) relation 
based analysis. 
Our analysis, given in algorithm \ref{alg:thread-modular}, entails interference combination $[\rf{a}{d}, \rf{b}{c}]$ to be infeasible, and therefore, can prove the property.
\begin{algorithm}
	\DontPrintSemicolon
	\LinesNumbered
	\SetKwFunction{FFeasInterf}{GetFeasibleInterfs}
	\SetKwFunction{FCP}{CartesianProduct}
	\SetKwFunction{FIsFea}{IsFeasible}
	\SetKwProg{Fn}{Function}{:}{}
	\SetKwData{LI}{LI} \SetKwData{AI}{AllInterfs}
	\KwData{$ \mathcal{T} $ is the set of threads in the program}
	\Fn{\FFeasInterf{$ \mathcal{T} $}} {
		$ \mathcal{IC} \leftarrow \phi $\;
		\ForEach{$ t \in \mathcal{T} $}{
			\ForEach{$ l \in \mathtt{Ld}_t $}{
				\LI(l) $ \leftarrow ctx $\;
				\ForEach{$ s \in  \mathtt{St}_{t'} $ for $ t' \neq t $}{
					\lIf{$ var(l) = var(s) $}{\LI $ \leftarrow $ \LI $ \cup\ \{s\} $ }
				}
			}
			\AI $ \leftarrow $ \FCP{\LI}\;
			\ForEach{$ i \in $ \AI }{
				\lIf{\FIsFea}{$ \mathcal{I}_f \leftarrow\mathcal{I}_f \cup \{i\} $}
			}
			$ \mathcal{IC} \leftarrow \mathcal{IC}[t \rightarrow \mathcal{I}_f] $
		}
		\KwRet{$ \mathcal{IC} $}
	}
	\caption{GetFeasibleInterferences}
	\label{alg:feas-interf}
\end{algorithm}

\subsection{Computing Interference Combinations} \label{subsec:interf-comb}
An interference combination $ \mathcal{IC}(t) $ for thread $ t $ consists of a set of reads-from relation for \emph{all} of its load instructions with \emph{some} store instruction of the different thread or current program state. 
We use reads-from relation of a load operation $ \ld $ with a special symbol $ ctx $ to denote that $ \ld $ is reading from current program state. 
In other words, an interference combination 
for thread $t$ is defined as $\mathcal{IC}(t): \{ \mathtt{Ld}_t \rightarrow ctx \cup (\bigcup\limits_{t' \neq t} \mathtt{St}_{t'}) \} $. 
Line 4-8 in algorithm \ref{alg:feas-interf} creates all such possible interference combinations for a thread $ t $.
%, $\mathcal{IC}: \mathcal{T} \rightarrow \{ic_1, ic_2, \mathellipsis \}$.

\subsection{Feasibility Analysis of Interference Combinations} \label{subsec:feasible}
We analysis each interference combination to check its feasibility under the semantics of the RA memory model.
This check is performed using \emph{reads-from} and \emph{sequenced-before} relations over the instructions involved in the interference combination. 
This feasibility check is done only once before starting the thread-modular analysis.

Our feasibility check uses the inference defined in figure \ref{fig:feas-rules} given immediate sequenced before information.
%We are using Z3 datalog engine to perform the analysis. 
%We encode Z3 with the immediate \emph{sequenced-before} instructions and inference rules \textsc{ppo, nrf1, nrf2, tcreate}  and \textsc{tjoin} given in figure-\ref{fig:feas-rules}. 
The \textsc{po, ppo, tcreate} and \textsc{tjoin} rules computes the entire \emph{ppo} set as shown in figure-\ref{fig:ex-trans-sb}. 
%Datalog engine uses rules \textsc{nrf1} (not-reads-from) and \textsc{nrf2} 
The rule \textsc{nrf} (not-reads-from) is used 
to find if the given interference combination is infeasible. 
If for any pair $ (s,l) $ in \emph{reads-from} relation (i.e., 
$ \rf{s}{l} $) in interference combination $ i_c $, the analysis infers 
$ \nrf{s}{l} $ ($ l $ cannot read from $ s $), the interference combination 
$ i_c $ is considered infeasible.

\begin{figure}[t]
	\begin{minipage}[b]{.31\textwidth}
		\centering
		\resizebox{.60\columnwidth}{!}{
			\input{figures/ex-trans-sb.tex}
		}
		\caption{Example of rule \textsc{ppo}}
		\label{fig:ex-trans-sb}
	\end{minipage}
	\begin{minipage}[b]{.31\textwidth}
		\centering
		\resizebox{.70\columnwidth}{!}{
			\input{figures/ex-nrf1.tex}
		}
		\caption{Example of rule \textsc{nrf}(1)}
		\label{fig:ex-nrf1}
	\end{minipage}
	\begin{minipage}[b]{.31\textwidth}
		\centering
		\resizebox{.70\columnwidth}{!}{
			\input{figures/ex-nrf2.tex}
		}
		\caption{Example of rule \textsc{nrf}(2)}
		\label{fig:ex-nrf2}
	\end{minipage}
\end{figure}

\begin{wrapfigure}{r}{0.37\textwidth}
\centering
%
\proofrule{tcreate}
{\lab:\tcreate{f}}{\ppo{\lab}{f.first}}

\proofrule{tjoin}
{\lab:\tjoin{f}}{\ppo{f.last}{\lab}}

\proofrule{po}{\seqb{op_1}{op_2}}{\ppo{op_1}{op_2}}

\proofrule{ppo}
{\ppo{op_1}{op_2} \qquad \ppo{op_2}{op_3}}
{\ppo{op_1}{op_3}}

\proofrule{nrf}
{\rf{s}{l} \qquad \ppo{l}{l'} \qquad \ppo{s'}{s}}
{\nrf{s'}{l'}}
%
%	\proofrule{nrf2}
%	{\rf{s}{l} \qquad \ppo{l}{l'}}
%	{\nrf{s}{l'}}
%
%	\proofrule{tcreate1}
%	{\lab:\tcreate{f} \qquad s \in f \qquad \seqb{l}{\lab}}{\nrf{s}{l}}
%	
%	\proofrule{tcreate2}
%	{\lab:\tcreate{f} \qquad l \in f \qquad \seqb{s}{\lab}}{\nrf{s}{l}}
%	
%	\proofrule{tjoin1}
%	{\lab:\tjoin{f} \qquad l \in f \qquad \seqb{\lab}{s}}{\nrf{s}{l}}
%	
%	\proofrule{tjoin2}
%	{\lab:\tjoin{f} \qquad s \in f \qquad \seqb{\lab}{l}}{\nrf{s}{l}}
%
\caption{Inference rules for Feasibility Analysis}
\label{fig:feas-rules}
\end{wrapfigure}

The feasibility check mitigates false positive on the example given 
in Figure-\ref{fig:why-ic}. 
If an instruction $s$ of thread $t_1$ interferes with an instruction $l$ of thread $t_2$, any later load $l'$ in $t_2$ cannot take its value from an instruction $s'$ that is ordered before $s$ in \emph{ppo}.
We have specified this constraint in inference rule \textsc{nrf} as shown in figure-\ref{fig:ex-nrf1}. 
%
Our semantics carry the entire dependence-before information of a store operation whenever a load operation reads from it. 
Hence, the interference of the form $ [\rf{s}{l}, \rf{s}{l'}] $ with $ \seqb{l}{l'} \orspace \seqb{l'}{l} $ is redundant. 
An example of such scenario is shown in figure-\ref{fig:red-interf}, where interference $ i_1 = [\rf{a}{b}, \rf{a}{c}] $ will be considered infeasible. 
Note that the states reachable using the interference $ i_1 $ are also be reachable using interference $ [\rf{a}{b}, \rf{ctx}{c}] $. 
Furthermore, if there is store operation $ \st $ in thread $ t_2 $ such that $ \seqb{b}{\st} \andspace \seqb{\st}{c} $, the interference $ i_1 $ will introduce imprecision in the set of reachable program states. 
Since the relation \emph{ppo} is reflexive the inference rule \textsc{nrf} marks such interferences infeasible as depicted in figure-\ref{fig:ex-nrf2}.

The time complexity of this check is $O(|i_c|^2\ .\ |ppo|^2)$, 
where $|i_c|$ is the size of interference combination (equals to the number of reads in the thread) and $|ppo|$ is the size of \emph{ppo} set (equals to the size of the thread). 
Using memoization, we can reduce the cost of querying \emph{ppo} to constant, reducing the cost of feasibility checking to $O(|i_c|^2)$.

\begin{lemma} \label{lem:infer-rules}
	The rules \textsc{tcretae, tjoin, po, ppo} and \textsc{nrf} do not infer any possibly feasible interference combination as infeasible.
\end{lemma}
%\begin{proof}
	Let some feasible interference combination $ i $ is marked as infeasible by our analysis.
	As defined in \textsection\ref{subsec:feasible}, it is possible only if a reads-from pair ($ \rf{s'}{l'} $) in the interference combination $ i $ is included in \emph{nrf} set by our analysis.
	The \textsc{tcreate, tjoin, po} and \textsc{ppo} rules are used to compute the  \emph{ppo} relation from immediate \emph{sequenced-before} information, rather than computing the relation \emph{nrf}. 
	Only rule \textsc{nrf} can entail that $ \nrf{s'}{l'} $. Hence, we will limit our discussion to rule \textsc{nrf} here.
	Since the rule \textsc{nrf} is marking $ \nrf{s'}{l'} $, $ \exists \rf{s}{l} \in i $ such that $ \ppo{l}{l'} $ and $ \ppo{s'}{s} $.
%	Remember that according to the semantics of the RA memory model, $ \setHB \defeq (\setSB \cup \setRF)^{+} $ and $ \setHB $ is irreflexive. 
	When $ s \neq s' $, an execution sequence that satisfies the premise of rule \textsc{nrf} cannot have irreflexive $ \setHB $, and therefore, is not a valid execution under the RA semantics.
	Hence the interference combination $ i $ is infeasible.
	Since our analysis carries entire information of a execution on any \emph{reads-from}, the information of $ \abs{\Sigma}(s) $ will be carried to instruction $ l $ if premise of rule \textsc{nrf} is satisfied and $ s = s' $. 
	Hence carrying it again at instruction $ l' $ will be same as another interference $ i' $ such that $ i' = i \setminus \{\rf{s'}{l'}\} \cup \{\rf{s'}{ctx}\} $. 
	Since our analysis is generating set of all possible interference combinations (as discussed in \textsection\ref{subsec:interf-comb}), the interference $ i $ becomes redundant, and hence, is safe to remove.
	Therefore, our analysis do not infer any possibly feasible interference combination as infeasible.
%\end{proof}

\begin{theorem}
	Our analysis is sound with respect to the RA semantics.
\end{theorem}
%\begin{proof}
	The soundness of our analysis follows from Lemma \ref{lem:infer-rules} and Theorem  \ref{thm:abspo-sound}. Theorem \ref{thm:abspo-sound} proves that under set of all possible interference combinations, our analysis is sound under the RA memory model. Lemma \ref{lem:infer-rules} proves that we are not pruning out any possibly feasible interference. Hence, our analysis is sound with respect to the RA semantics.
%\end{proof}


==> section/intro.tex <==
% Why are we interested in RA model
%% Analyzing parallel programs  under weakly consistent
%% memory models  is a challenging task.  
The difficulty in analysis of weak memory programs
arises from the fact that threads may
observe different values of program variables at a particular point in
time. The reordering of memory accesses performed by either the
compiler \cite{Batty-POPL12} or the hardware
\cite{popl-SarkarSNORBMA09}, and their runtime
interleavings is central to the variability in observation of program
memory states.
%
The problem only aggravates further when the weak memory model (\wmm)
under which a program executes cannot be reasoned with 
intuitive interleaving semantics.
%
One such memory model is the release-acquire (RA) fragment of the
 C/C++ 2011 standard~\cite{C11} (henceforth, referred to as the C11
 standard). In the RA model, all writes and reads are restricted to be
 {\em release} stores and {\em acquire} loads.
%
The RA model has been described in an {\em axiomatic} style where
program executions are defined as relations over {\em events}
mapping to program load/store and synchronization instructions. Typical
correctness in RA programs is defined by acyclicity axioms, which
can appear obscure. Such real and perceived difficulties necessitate the
development of automated analysis techniques to establish the
correctness of RA programs.
%

%
Notwithstanding its non-intuitive semantics, RA model is still one of
the cleaner subsets of the C11 standard with well-behaved semantics.
However, as noted before, RA programs can indeed produce
counter-intuitive outcomes that are unexplainable via reordering and
interleaving semantics.
%
%% It is worth noting that instruction-reordering and interleaving
%% semantics are some of the widely recognized ways through which one can
%% reason about the behaviors of \wmm programs. In the RA model,
%% however, due to the impositions placed by the release and
%% acquire semantics, the reordering of consecutive writes or reads
%% from a thread is disallowed. The behaviours of a program admitted
%% under RA model can indeed show counter-intuitive outcomes and may not
%% have an explanation via interleaving semantics alone.
%
Consider the example program (IRIW) \cite{LahavVafeiadis-POPL16} shown
with an example execution in Figure~\ref{fig:iriw-rel}.  
%% \begin{center}
%% \begin{tabular}{c||c||c||c c c}
%% $a: x \assign 1$ & $b: y \assign 1$ & $c: r_1 \assign x$ & $e: r_3 \assign y$ & & \\
%% &		 & $d: r_2 \assign y$ & $f: r_4 \assign x$ &  & \quad (IRIW)\\
%% \multicolumn{4}{c}
%% {$P: r_1==1 \andspace r_2==0 \andspace r_3==1 \implies r_4 \neq 0$} \\
%% \end{tabular}
%% \end{center}

\begin{figure}[!t]
\begin{minipage}{0.5\textwidth}
\centering
%\begin{adjustbox}{width=.65\textwidth,center}
%\fbox{
\input{figures/iriw-rel.tex}
%}
%\end{adjustbox}
\caption{IRIW execution  with {\em reads-from} (rf) and
{\em sequence-before} (sb) edges}
\label{fig:iriw-rel}	
\end{minipage}
%\vspace{-1em}
\hspace{1cm}
\begin{minipage}{0.4\textwidth}
		\centering
                %\begin{adjustbox}{width=.75\textwidth,center}
		%\fbox{
                \input{figures/ex2-rel.tex}
                %}
		%\end{adjustbox}
		\caption{HB relation via transitivity in (Trans-Dep)}
		\label{fig:ex2-rel}
	\end{minipage}
\end{figure}

If none of the reads were to be reordered, under the interleaving
semantics, the property 
$P: r_1==1 \andspace r_2==0 \andspace r_3==1 \implies r_4 \neq 0$
can never evaluate to false on systems that operate under memory
models such as SC, TSO (total store order) or PSO
(partial store order). 
%% One would have expected that in the RA model,
%% due to the absence of reordering of consecutive read acquires, the
%% assertion to remain inviolable.
However, under RA semantics, no guarantee of a total order on the global visibility of
writes observed at labels {\tt a} and {\tt b} is provided, thus $P$ can evaluate to false.
The assertion-violating
execution for (IRIW) is shown in Figure~\ref{fig:iriw-rel}. %% It
%% is noteworthy that such a behavior cannot be explained either by
%% interleaving semantics or via instruction reorderings, thus,
%% disallowed under SC, TSO and PSO models


Nonetheless, there are some fascinating aspects of RA semantics.
Under the RA model, a total order on all the writes to the same global
variable is enforced. More importantly, when a load instruction of a thread
$t$ observes (or {\em synchronizes} with) a store from another thread
$t'$, then all the prior writes observed by $t'$ up to the
synchronizing store operation also become observable to $t$.
%
In other words, a reading thread inherits the program state (as a
valuation of global variables) that was available to the writing
thread just before the point of
synchronization. It is worth noting that these aspects make RA
semantics naturally amenable for {\em localized} or {\em
thread-modular} reasoning, which is a
well-considered area of research. 

% What is prior thread-modular work for rmm and RA programs?
Thread-modular approaches broadly function in two steps, which is also
the basis of the {\em rely-guarantee} proof
technique~\cite{Jones1981DevelopingMF}.  In the first step, each
thread in the program is analyzed in isolation, and a set of invariants
(called {\em guarantees}) over the global environment is computed that
the thread cannot violate.
%
In the second step, each thread is analyzed again taking into account 
the guarantees of other threads. If any change to the thread's
set of invariants is discovered the entire process is repeated.
%
As a model checking approach applied to SC programs, the thread-modular
technique was first proposed in~\cite{Flanagan-SPIN03}.
%
In the recent past, several contributions 
\cite{SuzanneMine-APLAS18,Mine-VIMCAI17,SuzanneMine-SAS16,KusanoWang-FSE16,KusanoWang-FSE17}
have been presented (in the context of verifying \wmm programs)
where sequential abstract interpreters were
bootstrapped with thread-modular reasoning. 
% to verify \wmm programs.
%% The above contributions have been largely thread-modular (with the
%% exception of \cite{farzan_duet_2013}) in their approach.

%
%
Techniques such as in~\cite{SuzanneMine-SAS16,SuzanneMine-APLAS18}
analyze \wmm programs by fundamentally relying on a model of store
buffers. Evidently, RA program behaviors 
cannot be simulated using store buffers \cite{LahavVafeiadis-POPL16}.
Thus, the above-mentioned contributions cannot be generalized to
reason about RA semantics without re-modeling for the operational
semantics of RA~\cite{KangVafeiadis-POPL17}.
%
Furthermore, flow- and context-sensitivity based thread-modular
abstract interpretation (TMAI) techniques in \textsc{Watts} and
\textsc{FruitTree}~\cite{KusanoWang-FSE17,KusanoWang-FSE16} do not capture
ordering constraints among a set of instructions involving more than
two threads. Consider the example (Trans-Dep) shown below. \\ 
%\begin{minipage}{0.49\linewidth}
%\centering
%% \begin{center}
%% \begin{tabular}{c||c||cc}
%% %\multicolumn{3}{c}{(Trans-Dep)} \\
%% $a: x \assign 1$ & $b: r_1 \assign x$ & $d: r_2 \assign x$ &  \\
%%            & $c: x \assign 2$ & $e: r_3 \assign x$ &\quad (Trans-Dep)\\
%% %\multicolumn{3}{c} {$P_1: r_1==1 \andspace r_2==2 \implies r_3\neq 2$ \divya{invalid}} \\
%% \multicolumn{3}{c} {$P: r_1==1 \andspace r_2==2 \implies r_3==2$} 
%% \end{tabular}
%% \end{center}
%\end{minipage}
%% \begin{minipage}[c]{0.49\linewidth}
%% \centering
%% \begin{tabular}{c||c}
%% \multicolumn{2}{c}{(Simp-2W2R)} \\
%% $a: x = 1$ &$c: r_1 = y$ \\
%% $b: y = 1$ &$d: r_2 = x$ \\
%% \multicolumn{2}{c} {$P_{true}: r_1=1 \implies r_2=1$} \\
%% \end{tabular}
%% \end{minipage}
Property $ P $ in (Trans-Dep) example can be proved only
if the inter-thread dependencies among all the three threads are captured. In
particular, when $r_1 == 1 \wedge r_2 == 2$, there is an ordering
relation from $a$ to $e$ (as shown in Figure~\ref{fig:ex2-rel})
which cannot be computed with the {\tt po} and {\tt rf}
relations alone while considering only two threads at a
time. {\sc FruitTree} fails to prove the above
property.
%

%
Other works \cite{Gavrilenko-CAV19,AbdullaKrishna-PLDI19} use bounded
model checking techniques (BMC) to verify programs under weak memory
semantics. However, such techniques provide sound results only under
the bound in which they are operating. A detailed discussion on recent
advances on BMC techniques and how our work is positioned {\em vis-\`a-vis} them
is provided in \textsection\ref{sec:related-work}.

%% List of contributions
\noindent{\bf Contributions and Outline}:
In our observations, none of the above discussed TMAI techniques so
far can reason about RA programs in an automated manner.
%% Table~\ref{table:tool-overview}
%% presents an overview of sound static methodologies and associated
%% tools in the design space of verification for \wmm programs.
%  
In this paper, we propose a TMAI technique (see \textsection\ref{sec:thr-mod})
for RA programs using novel
partial order based abstract domains.
%
%% Not only do we tailor the thread-modular abstract interpretation for
%% RA memory model constraints, we use these constraints innovatively as
%% a light-weight mechanism to capture the set of feasible execution
%% environments, thus, lending some degree of flow-sensitivity to our
%% analysis.
%
The notion of using partial orders to analyze program executions is
well known, and indeed many prior works have exploited this idea. %%  For
%% instance, \cite{KokologiannakisVafeiadid-POPL18} uses partial orders
%% that include {\tt rf} and {\tt ppo} (preserved program order) to
%% analyze a repaired version of C11 model, and \cite{AlglaveKT13}
%% provided partial order encodings for \wmm programs operating under the
%% hood of a bounded model checker. 
We present a detailed summary of
such work in \textsection\ref{sec:related-work}.
%
%
%
However, we use partial orders in a novel way --  as abstract domains to
represent abstract program semantics (see \textsection\ref{sec:abs-sem}).
The starting point in our analysis is the modeling of concrete program
semantics as a set of total orders on writes per global variable, also
known as {\em modification orders} ({\tt
mo})(see \textsection\ref{sec:con-sem}). In turn a collection of
modification orders can be collectively represented as a partial
order.
%% (as long as {\em consitency} requirement is
%% met, \textsection\ref{sec:}).
%
A combination of variables' value abstraction (using numerical or
relational abstract domains) along with the abstraction of the global
environment (using partial orders) forges the foundation of our
analysis.
%
It is worth noting that the use of partial orders as
an abstract domain has general applicability,
and could be applied to other memory models too (see \textsection\ref{sec:mo-po-lat}).
%
We abstract further the {\tt mo}-specific partial orders by only preserving the {\em latest
writes} per thread per variable in the partial order and forgetting
all older writes. This abstraction is specific to the RA memory model.
We show that this {\em abstract upper approximation}
does not alter the correspondence between the concrete and abstract domains  (see \textsection\ref{sec:abs-sem}).

%
%
Furthermore, to establish that our analysis preserves soundness and is
terminating, we show that (i) the lattice corresponding to the
abstract semantics is {\em complete}, (ii) establish
a  {\em Galois connection} between the concrete and abstract
domains, and (iii) prove that the {\em abstract upper approximation} is
sound with respect to RA semantics. %% The
%% certainty of the existence of a {\em least fixed point} ({\tt lfp}) in
%% our analysis is ensured by the {\em Knaster-Tarski} theorem.
%
%% Our technique explores all relevant, reachable abstract states of the
%% program when the above-discussed computation steps reach a fix point.
%
Finally, we implement our proposed analysis in a tool called \tool and
demonstrate its effectiveness by comparison with a recent (and the only
other auotmatic tool to verify RA programs) BMC
tool \cite{AbdullaKrishna-PLDI19} that can analyze RA programs
(see \textsection\ref{sec:experiments}).

% The main contributions of this paper in summary are: (C1) 
In  \textsection\ref{sec:ovw}, we present a
detailed intuitive account of our contributions through examples
before presenting the theoretical underpinnings of \tool.




% Overview of our technique. 
%% 


%\captionsetup[figure]{font=footnotesize}
%% \begin{figure}[!t]
%% 	\begin{minipage}{0.49\textwidth}
%% 	\centering \footnotesize
%% 	\fbox{\begin{tabular}{c||c||c}
%% 		$a: x=1$ & $b: r_1=R(x)$ & $d: r_2=R(x)$ \\
%% 			 & $c: y = r_1$  & $e: r_3=R(y)$ \\
%% 		\multicolumn{3}{c} {$P_{false}: r_2 \neq 1 \orspace r_3 \neq 1 $} \\
%% 	\end{tabular}}
%% 	\caption{Modified 1W2R}
%% 	\label{fig:vbmc-no-bug}
%% 	\end{minipage}
	%% \begin{minipage}{0.49\textwidth}
	%% 	%\newcolumntype{C}{>{\centering\arraybackslash}p{6em}}
	%% 	\footnotesize \centering
	%% 	\fbox{
	%% 		\begin{tabular}{c||c||c||c}
	%% 			$a: x = 1$ & $b: y = 1$ & $c: r_1=R(x)$ & $e: r_3=R(y)$ \\
	%% 			&		 & $d: r_2=R(y)$ & $f: r_4=R(x)$ \\
	%% 			\multicolumn{4}{c}
	%% 			{$P_{false}: r_1=1 \andspace r_2=0 \andspace r_3=1 \implies r_4 \neq 0$} \\
	%% 	\end{tabular}}
	%% 	\caption{IRIW example}
	%% 	\label{fig:iriw-ex}
	%% \end{minipage}
%% \end{figure}


%\begin{figure}
%%	\begin{minipage}{.40\textwidth}
%	\centering \tiny
%	\fbox{\begin{tabular}{l||l||l||l}
%			$a: x=1$ & $b:$ if $R(x)$  		 & $f: r_2=R(z)$ & $i: z=1$\\
%					 & $c: \hspace{1em} x=2$ & $g: r_3=R(y)$ & \\
%					 & $d: \hspace{1em} y=2$ & $h: r_4=R(x)$ & \\
%					 & $e: \hspace{1em} r_1=R(z)$ &  & \\
%			\multicolumn{4}{c} {$P_{true}: r_3=2 \implies r_4=2 $} \\
%			\multicolumn{4}{c} {$P_{false}: r_1=0 \andspace r_2=0 \implies r_4 \neq 0 $} \\
%	\end{tabular}}
%	\caption{Running Example: ???}
%	\label{fig:running-ex}
%%	\end{minipage}
%\end{figure}

%\begin{figure}
%	\centering
%	\newcolumntype{C}{>{\centering\arraybackslash}p{2cm}}
%	\begin{tabular}{C||C}
%		$a: z = R(x)$ & $d: y = 1$ \\
%		$b: y = 2$ 	  & $e: x = 1$ \\
%		$c: x = 2$    & $f: a = R(x)$ \\
%					  & $g: b = R(y)$ \\
%					  & $h: c = R(z)$ \\
%		\multicolumn{2}{c} {assert $(a \neq 2 \orspace c \neq 1 \orspace b \neq 2)$} \\
%	\end{tabular}
%	\caption{VBMC can't catch bug with K=2}
%	\label{fig:vbmc-no-bug}
%\end{figure}



%
%% \begin{table}
%% 	\centering
%% %	\scriptsize
%% 	\footnotesize
%% 	\begin{tabular}{ccc@{\hskip 6pt}c}
%% 		\toprule
%% 		Tool 	& Type  	& State Space & RA behaviors \\
%% 		\midrule
%% 		\textsc{Tracer}\cite{Abdulla-OOPSLA2018} 	& Dynamic 	& \xmark & \cmark \\
%% 		\textsc{VBMC}\cite{AbdullaKrishna-PLDI19}	& View-Bounding & \xmark & \cmark \\
%% %		\textsc{Watts}	& TMAI & \cmark & \xmark \\
%% 		\textsc{FruitTree}\cite{KusanoWang-FSE17}	& TMAI & \cmark & \xmark \\
%% 		Batman\cite{Mine-VIMCAI17}	& TMAI & \cmark & \xmark \\
%% 		SuzanneMine\cite{SuzanneMine-APLAS18} & TMAI & \cmark & \xmark \\
%% %		SuzanneMineRelational & TMAI & \cmark & \xmark \\
%% 		\textsc{Dartagnan}\cite{Gavrilenko-CAV19} & BMC & \xmark & \xmark \\
%% 		\textsc{Duet}\cite{Farzan-POPL12,farzan_duet_2013} & AI & \cmark & \xmark \\
%% 		\bottomrule
%% 		\multicolumn{4}{c}{\rule[.25cm]{0pt}{0cm} \scriptsize TMAI: Thread-Modular Abstract Interpretation}
%% 	\end{tabular}
%% 	\caption{Overview of Existing Tools}
%% 	\label{table:tool-overview}
%% \end{table}
%% Thus, as the focus of this study, we choose
%% to develop an automatic reasoning approach for RA programs.
%
% What is this study's objective
%% In this work, we present an automated method to statically verify
%% RA programs for reachability properties; in particular, properties
%% that are specified as assertion statements in a program at definite
%% control locations. We establish our method to be sound with guaranteed
%% termination. 
%


==> section/new-approach.tex <==
% what is new approach
The partial order domain proposed in \textsection \ref{subsec:con-po-mo} 
incorporates the information of current execution. A careful reader might 
observe that consistency ($ \iscons $) and extensibility ($ \isext $) checks 
are sufficient to prune out infeasible executions. In fact, slight changes in 
these checks and along with the semantics of $ \ld/\st/\rmw $ operations is 
can suffice to make the approach applicable for other non-atomic memory models 
as well \divya{we need to rethink about this. How can we prove this claim, if true?}. 

Hence, we extend our approach to consider interferences for each read 
operation individually rather than using interference combinations. A load 
operation can read-from either latest write in the current thread or a write 
form other thread. Hence, we define our interferences as a set of map from 
each read operation in the program to a set of write operations. Same as our 
previous approach, we use $ ctx $ to define read from current context 
(latest write in current thread). Formally, set of interference $ 
\mathcal{I}: \mathtt{Ld} \rightarrow \{ctx \cup (\bigcup\limits_{t' \neq t} 
\mathtt{St}_{t'})\} $

% algorithm and explaination
\begin{algorithm}
	\DontPrintSemicolon
	\LinesNumbered
	\SetKwFunction{FThrMod}{ThreadModularAnalysis2}
	\SetKwFunction{FSeqAbsMod}{SeqAIModified}
	\SetKwProg{Fn}{Function}{:}{}
	\KwData{$ \mathcal{T} $ is the set of threads in the program}
	\Fn{\FThrMod{$ \mathcal{T} $}} {
		\tcp{Intialization}
		%		$ \Sigma \leftarrow \phi $\;
		$ \sigma \leftarrow \phi $\;
		\Repeat(\tcp*[f]{fix-point iteration}){$ \Sigma = \sigma $}{
			$ \Sigma \leftarrow \sigma $\;
			\ForEach{$ t \in \mathcal{T} $}{
				$ \sigma \leftarrow \sigma\ \uplus\ $\FSeqAbsMod{$ t, \Sigma, i $}
			}
		}
	}
	\caption{ThreadModularAnalysis2}
	\label{alg:thread-modular2}
\end{algorithm}

The algorithm \texttt{SeqAIModified} given in \ref{alg:seq-abs-mod} remains same with change in signature of interference $ i $, which will be passed to $ \semof{} $ operator. The modifications to $ \semof{} $ operators are given in  figure \ref{fig:sem-updated}.
We update algorithms \ref{alg:thread-modular} to accommodate required changes for this analysis. The modified algorithm is shown in ... \divya{Only changes are deletion of line number 3 and loop in line 7. How to write it properly}

\begin{figure}
	\centering
	\begin{align}
	\begin{split} \label{eq:ld-updated}
	\MoveEqLeft[3] \semof{\lab: \load{x}} (\Sigma, i) \defeq \\
	& \assume \sigma=\phi \\
	& \modified{\forall \st \in i(\lab),} \\
	& \forall(l, mo_l, m_l) \in \Sigma(pre(\lab)), (s, mo_s, m_s) \in \Sigma(\st)\ .\ mo_l \iscons mo_s \andspace mo_l \isext \st \implies \\
	& \quad \assume mo' = (mo_l \join mo_s) \append \st \andspace m''=m_l \join m_s \andspace m' = m''[x \rightarrow m_s(x)]  \\
	& \quad \inn \sigma\ \modified{\join}= (\lab, mo', m') \\
	& \inn  \{\sigma/\Sigma(\lab)\}\Sigma
	\end{split}
	\end{align}
	\caption{Concrete Semantics of the RA programs}	
	\label{fig:sem-updated}
\end{figure}

% modified semantics of load operation
Since interferences effect $ \ld $ and $ \rmw $ operations, the semantics of 
these operations are changed with changes in definition of interference.
The semantics of $ \rmw $ operations defined in \ref{eq:con-rmw} uses $ \ld $
operation. Hence, updating semantics of only $ \ld $ operation will suffice our purpose. The changes are highlighted in \modified{red} color in equation \ref{eq:con-ld}. The first change is to use all the store operations in set $ i(\lab) $. The second change is using operator $ \join $ to join the environment with already existing one. The operator $ \join $ here joins two $ m_1 $ and $ m_2 $ whenever $ mo_1 = mo_2 $. 


==> section/ra-formal.tex <==
An event $ e $ is some operation over $ \mathit{Var}(e)\in \vars $.

\begin{align*}
 \MoveEqLeft[3] \vse{a}{b} \defeq \hb{a}{b} \andspace 
	a \in \mathtt{St} \cup \mathtt{RMW} \andspace
	b \in \mathtt{Ld} \andspace 
	\mathit{Var}(a) == \mathit{Var}(b) \andspace \\
& \neg (\exists c .\ c \neq a \andspace c \neq b \andspace 
	c \in \mathtt{St} \cup \mathtt{RMW} \andspace 
	\mathit{Var}(c) == \mathit{Var}(b) \andspace
	\hb{a}{c}\hb{}{b} )
\end{align*}
$ \vse{a}{b} $ implies there is no store $ c $ happens-after store $ a $ and happens-before load $ b $.

\begin{align*}
\MoveEqLeft[5] \text{consistent\_modification\_order} \defeq \\
\MoveEqLeft[3] (\forall a.\ \forall b.\ \edgeMO{a}{b} \implies 
\mathit{Var}(a) == \mathit{Var}(b)) \andspace 
%\MoveEqLeft[2] 
(\forall v \in \vars \\ 
	\MoveEqLeft[1] \assume actions\_at\_v = \{a.\ \mathit{Var}(a) == v\}\ \inn \\
	\MoveEqLeft[1] \assume stores\_at\_v == \{a \in actions\_at\_v 
	\andspace a \in (\mathtt{St} \cup \mathtt{RMW}) \}\ \inn \\
	& \text{strict\_total\_order\_over}\ stores\_at\_v  (\edgeMO{}{}|_{actions\_at\_v} ) \andspace \\
	& \hb{}{}|_{stores\_at\_v} \subseteq 
	\edgeMO{}{}|_{actions\_at\_v} ) 
\end{align*}
$ \setMO $ is a strict total order over all stores/rmw events of a 
variable and it is consistent with $ \setHB $.

Let $ \mathit{Tid}(e) $ is the thread id of an event $ e $.
\begin{align*}
\text{rs\_element}\ rs\_head \ a \defeq 
(\mathit{Tid}(a) ==  \mathit{Tid}(rs\_head)) \orspace 
a \in \mathtt{RMW}
\end{align*}
\begin{align*}
\MoveEqLeft[3] \relseq{a}{b} \defeq \\
	\MoveEqLeft[1] a \in (\mathtt{St} \cup \mathtt{RMW}) \andspace ((b==a) \orspace  \\
	 \MoveEqLeft[1] (\text{rs\_element}\ a \ b \andspace \edgeMO{a}{b} \ \andspace 
	 (\forall c.\ \edgeMO{a}{c}\edgeMO{}{b} \implies 		\text{rs\_element}\ a \ c )))
\end{align*}
A \emph{release sequence} is  a contiguous subsequence of modification order starting from a release stores and followed by any stores from the same thread or rmw from any thread.

\begin{align*}
\MoveEqLeft[3] \sw{a}{b} \defeq \\
	\MoveEqLeft[1] \text{(*additional synchronizes with from thread create, join etc *)} \\
	\MoveEqLeft[1] a \xrightarrow{\mathit{asw}} b \orspace \\
	\MoveEqLeft[1] (\mathit{Var}(a) == \mathit{Var}(b) \andspace ( \\
	& \text{(* mutex synchronization *)} \\
	& (a \in \mathtt{Unlock} \andspace b \in \mathtt{Lock} \andspace 
		\hb{a}{b}) \orspace \\
	& \text{(* RA synchronization *)} \\
	& (a \in (\mathtt{St} \cup \mathtt{RMW}) \andspace 
		b \in (\mathtt{Ld} \cup \mathtt{RMW}) \andspace 
		\neg(\mathit{Tid}(a) ==  \mathit{Tid}(b)) \andspace \\
		& (\exists c.\ \relseq{a}{c}\rf{}{b}	 ) )  )
\end{align*}
An event $ a $ synchronizes-with another $ b $ if any of the following satisfies:
\begin{enumerate}
	\item $ a $ additionally-synchronizes-with $ b $. Events such as thread create and join induce additionally-synchronizes-with. 
	\item $ a $ is an mutex unlock that happens-before mutex lock $ b $.
	\item $ a $ is a release store or rmw synchronizes-with a load or rmw  $ b $ from different thread if $ b $ reads from some store in the release sequence of $ a $
\end{enumerate}

\begin{align*}
\MoveEqLeft[3] \text{visible\_sequence\_of\_side\_effects}\ vsse\_head \ b \defeq \\
	& \{c.\ \edgeMO{vsse\_head}{c} \andspace \neg(\hb{b}{c}) \andspace \\ 
	& (\forall a.\ \edgeMO{vsse\_head}{a}\edgeMO{}{c} \implies 
	\neg(\hb{b}{a}) )  \}
\end{align*}
For any load, visible-sequence-of-side-effects is a set of continuous 
sub-sequence of modification order headed by visible side effect to the 
load, where the load does not happen before any event in the sequence.
A load or rmw must read from a store or rmw in it's 
visible-sequence-of-side-effects set.
